Stock Market Telepathy: Graph Neural Networks Predicting the Secret Conversations between MINT and G7 Countries

Emerging economies, particularly the MINT countries (Mexico, Indonesia, Nigeria, and T\"urkiye), are gaining influence in global stock markets, although they remain susceptible to the economic conditions of developed countries like the G7 (Canada, France, Germany, Italy, Japan, the United Kingdom, and the United States). This interconnectedness and sensitivity of financial markets make understanding these relationships crucial for investors and policymakers to predict stock price movements accurately. To this end, we examined the main stock market indices of G7 and MINT countries from 2012 to 2024, using a recent graph neural network (GNN) algorithm called multivariate time series forecasting with graph neural network (MTGNN). This method allows for considering complex spatio-temporal connections in multivariate time series. In the implementations, MTGNN revealed that the US and Canada are the most influential G7 countries regarding stock indices in the forecasting process, and Indonesia and T\"urkiye are the most influential MINT countries. Additionally, our results showed that MTGNN outperformed traditional methods in forecasting the prices of stock market indices for MINT and G7 countries. Consequently, the study offers valuable insights into economic blocks' markets and presents a compelling empirical approach to analyzing global stock market dynamics using MTGNN.

==> preamble.tex <==
\usepackage[table,x11names,svgnames,dvipsnames]{xcolor}
\usepackage[export]{adjustbox}
% \usepackage{algorithm}
% \usepackage[noend]{algpseudocode}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage[USenglish]{babel}
\usepackage{bigints}
\usepackage{bm}
\usepackage{booktabs}
\usepackage{cancel}
\usepackage[tableposition=above, font=normalsize]{caption}
% \usepackage{centernot}
% \usepackage{comment}
\usepackage{enumitem}
\usepackage{epsfig}
\usepackage{epstopdf}
% \epstopdfsetup{outdir=./figures//}
% \usepackage[letterpaper, top=1.0in, bottom=1.0in, left=1.0in, right=1.0in]{geometry}
\RequirePackage[OT1]{fontenc}
% \usepackage{fontspec}
\usepackage{graphics}
\usepackage{graphicx}
\graphicspath{{../figures/}}
% \usepackage{ifpdf}
% \usepackage{lastpage}
% \usepackage{leftidx}
\usepackage{lineno}
\usepackage{lipsum}
% \usepackage{mathrsfs}
\usepackage{mathtools}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{nicefrac}
% \usepackage{nicematrix}
% \usepackage{pgfplots}
\usepackage{pifont}
% \usepackage{ragged2e}
% \usepackage{rotating}
% \usepackage{stmaryrd}
\usepackage{siunitx}
\usepackage{soul}
\usepackage[caption=false]{subfig}
\usepackage{tabularx}
\usepackage{threeparttable}
\usepackage{tikz}
% \usepackage{tkz-euclide}
% \usepackage{ctable}
% \usetikzlibrary{matrix, arrows}
\usetikzlibrary{shapes.geometric, arrows, decorations.markings, shapes.arrows}

\newcommand{\minitab}[2][l]{\begin{tabular}{#1}#2\end{tabular}}

%%%%%%% TODO NOTES 
\usepackage{todonotes}
\setlength{\marginparwidth}{1.3cm}
\setlength{\marginparsep}{0cm}
\newcommand{\ctodo}[1]{\todo[size=\tiny]{#1}}
\newcommand{\nnparam}{\theta}
\newcommand{\pinn}{\pi_{\nnparams}}

\usepackage{wrapfig}

\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=1cm, minimum
height = 0.5cm, text centered, draw=black, fill=red!30]
\tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110,
minimum height=1cm, text width=3cm, text centered, draw=black, fill=blue!30]
\tikzstyle{process} = [rectangle, minimum width=2cm, minimum height=0.8cm, text
centered, text width=2cm, draw=black, fill=orange!30]
\tikzstyle{decision} = [diamond, aspect=1.25, minimum width=2cm, minimum height=0.5cm, 
text centered, text width=3cm, draw=black, fill=green!30]
\tikzstyle{arrow} = [thick, ->, >=stealth]




\makeatletter
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother

\newcommand{\bmat}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\pmat}[1]{\begin{pmatrix}#1\end{pmatrix}}
\newcommand{\ubar}[1]{\text{\b{$#1$}}}
\newcommand{\norm}[2]{\|{#1}\|_{{}_{#2}}}
\newcommand{\abs}[1]{\left|{#1}\right|}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\dd}{\operatorname{d}\!}
\newcommand{\muc}[2]{\multicolumn{#1}{c}{#2}}
\newcommand*\Eval[3]{\left.#1\right\rvert_{#2}^{#3}}
\newcommand{\inner}[1]{\left\langle#1\right\rangle}
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdd}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\el}[2]{\frac{\dd}{\dd t}\pd{\mc{L}}{\dot{#1}} - \pd{\mc{L}}{#1} = #2}
\newcommand{\elk}[2]{\frac{\dd}{\dd t}\pd{\mc{L}}{\dot{#1}_k} - \pd{\mc{L}}{#1_k} = #2_k}
\newcommand{\vectornorm}[1]{\left|\left|#1\right|\right|}
\newcommand{\dom}[1]{\textrm{dom}\;#1}
\newcommand{\bx}{{\bf x}}
\newcommand{\bu}{{\bf u}}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand*{\vertbar}{\rule[-1ex]{0.5pt}{2.5ex}}
\newcommand*{\horzbar}{\rule[.5ex]{2.5ex}{0.5pt}}

\newcommand{\idapbc}{\textsc{IdaPbc}}
\newcommand{\electric}{{\textcolor{blue}{\hspace{-0.5mm}$\bm{E}$\;}}}
\newcommand{\magnetic}{{\textcolor{red}{\hspace{-0.5mm}$\bm{B}$\;}}}

% \theoremstyle{plain}
% \newtheorem{thm}{Theorem}[section]
\newtheorem{thm}{Theorem}
% \makeatletter
% \@addtoreset{thm}{section}
% \makeatother
% \newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}{Lemma}
% \newtheorem{claim}[thm]{Claim}
% \newtheorem{axiom}[thm]{Axiom}
% \newtheorem{conj}[thm]{Conjecture}
% \newtheorem{fact}[thm]{Fact}
% \newtheorem{hypo}[thm]{Hypothesis}
% \newtheorem{assum}[thm]{Assumption}
\newtheorem{prop}{Proposition}
% \newtheorem{crit}[thm]{Criterion}
% \theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
% \newtheorem{exmp}[thm]{Example}
\newtheorem{rem}{Remark}
% \newtheorem{prin}[thm]{Principle}

\DeclareMathOperator{\Tr}{tr}
\newcommand\xdownarrow[1][2ex]{%
   \mathrel{\rotatebox{90}{$\xleftarrow{\rule{#1}{0pt}}$}}
}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\vers}{vers}
\DeclareMathOperator{\trans}{Trans}
\DeclareMathOperator{\rot}{Rot}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\sinc}{sinc}

\usepackage{hyperref}
\hypersetup{
    unicode=false,          % non-Latin characters in Acrobat’s bookmarks
    pdftoolbar=true,        % show Acrobat’s toolbar?
    pdfmenubar=true,        % show Acrobat’s menu?
    pdffitwindow=false,     % window fit to page when opened
    pdfstartview={FitH},    % fits the width of the page to the window
    pdftitle={Stock Market Telepathy: Graph Neural Networks Predicting the Secret Conversations between MINT and G7 Countries},    % title
    pdfauthor={Nurbanu Bursa}, % author
    % pdfsubject={Subject},   % subject of the document
    % pdfcreator={Creator},   % creator of the document
    % pdfproducer={Producer}, % producer of the document
    % pdfkeywords={keyword1, key2, key3}, % list of keywords
    pdfnewwindow=true,      % links in new PDF window
    colorlinks=true,       % false: boxed links; true: colored links
    linkcolor=blue!30!green,          % color of internal links (change box color with linkbordercolor)
    linkbordercolor=orange,
    citecolor=blue,        % color of links to bibliography
    citebordercolor=green,
    filecolor=magenta,      % color of file links
    urlcolor=cyan,           % color of external links
    urlbordercolor=blue,
}

